Group Fairness by Probabilistic Modeling with Latent Fair Decisions

Machine learning systems are increasingly being used to make impactful decisions such as loan applications and criminal justice risk assessments, and as such, ensuring fairness of these systems is critical. This is often challenging as the labels in the data are biased. This paper studies learning fair probability distributions from biased data by explicitly modeling a latent variable that represents a hidden, unbiased label. In particular, we aim to achieve demographic parity by enforcing certain independencies in the learned model. We also show that group fairness guarantees are meaningful only if the distribution used to provide those guarantees indeed captures the real-world data. In order to closely model the data distribution, we employ probabilistic circuits, an expressive and tractable probabilistic model, and propose an algorithm to learn them from incomplete data. We evaluate our approach on a synthetic dataset in which observed labels indeed come from fair labels but with added bias, and demonstrate that the fair labels are successfully retrieved. Moreover, we show on real-world datasets that our approach not only is a better model than existing methods of how the data was generated but also achieves competitive accuracy.

==> tikzlibraryspn.code.tex <==
% Copyright 2016 by Nicola Di Mauro and Antonio Vergari
%
% This file may be distributed and/or modified
%
% under the GNU General Public License.
%
% See the files LICENSE for more details.

\usetikzlibrary{chains}
%\usetikzlibrary{arrows}
\usepackage{pgfplots}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}

% sum node style
\tikzstyle{sum} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.west) -- (path picture bounding box.east);}, node distance=1]

% product node style
\tikzstyle{prod} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south east) -- (path picture bounding box.north west); \draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south west) -- (path picture bounding box.north east);}, node distance=1]

% \sumnode [tikz-options] {sum node name} 
\newcommand{\sumnode}[2][]{
  \node[sum, #1] (#2) {};
}

% \prodnode [tikz-options] {product node name} 
\newcommand{\prodnode}[2][]{
  \node[prod, #1] (#2) {$\times$};
}
\newcommand{\wprodnode}[3][]{
  \node[prod, #1] (#2) {$\color{#3}\times$};
}

% \maxnode [tikz-options] {max node name} 
\newcommand{\maxnode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {\scriptsize $max$};
}

% \emptynode [tikz-options] {generic node name}
\newcommand{\emptynode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {};
}

\newcommand{\varnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\varsqnode}[4][]{
  \node[rectangle, rounded corners=3pt,fill=white,draw=#4,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\evnode}[4][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt, #1] (#2) {#3};
}

\newcommand{\evnodevar}[5][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt,
  #1] (#2) {#3};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#5};
}

\newcommand{\bernode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\contnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\catnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] coordinates { (0,0) (0,10)};
                \addplot [mark=none] coordinates { (-1,0) (-1,7)};
                \addplot [mark=none] coordinates { (-2,0) (-2,3)};
                \addplot [mark=none] coordinates { (1,0) (1,5)};
                \addplot [mark=none] coordinates { (2,0) (2,8)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2] (#2_vn) {#3};
}


% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;%
    } ;
  } ;
}

\newcommand{\upedge}[3][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1] (#3);
}

\newcommand{\ledge}[4][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1,edge label=#4] (#3);
}

\newcommand{\weigedge}[4][]{
  \draw[line width=0.6pt,-,#1] (#2) edge node [midway,line width=0.6pt,#1] {#4} (#3) ;
}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

